High Performance Data Persistence in Non-Volatile Memory for Resilient High Performance Computing

Resilience is a major design goal for HPC. Checkpoint is the most common method to enable resilient HPC. Checkpoint periodically saves critical data objects to non-volatile storage to enable data persistence. However, using checkpoint, we face dilemmas between resilience, recomputation and checkpoint cost. The reason that accounts for the dilemmas is the cost of data copying inherent in checkpoint. In this paper we explore how to build resilient HPC with non-volatile memory (NVM) as main memory and address the dilemmas. We introduce a variety of optimization techniques that leverage high performance and non-volatility of NVM to enable high performance data persistence for data objects in applications. With NVM we avoid data copying; we optimize cache flushing needed to ensure consistency between caches and NVM. We demonstrate that using NVM is feasible to establish data persistence frequently with small overhead (4.4% on average) to achieve highly resilient HPC and minimize recomputation.

==> text/impl.tex <==
\section{Implementation (0.5 page)}
\label{sec:impl}
